Decoding Holographic Codes with an Integer Optimisation Decoder

We develop a most likely error Pauli error decoding algorithm for stabiliser codes based on general purpose integer optimisation. Using this decoder we analyse the performance of holographic codes against Pauli errors and find numerical evidence for thresholds against Pauli errors for bulk qubits. We compare the performance of holographic code families of various code rates and find phenomenological Pauli error thresholds ranging from $7\%$ to $16\%$, depending on the code rate. Additionally we give numerical evidence that specific distance measures of the codes we consider scales polynomially with number of physical qubits.

==> HeptagonCodePauli.tex <==
% !TEX root = Master.tex
 




  \title{Decoding Holographic Codes with an Integer Optimisation Decoder}
  \author{Robert J. Harris}
  \email{rjh2608@gmail.com}
\affiliation{ARC Centre for Engineered Quantum Systems, School of Mathematics and Physics, The University of Queensland, St Lucia, QLD, 4072, Australia}
\author{Elliot Coupe}
\affiliation{ARC Centre for Engineered Quantum Systems, School of Mathematics and Physics, The University of Queensland, St Lucia, QLD, 4072, Australia}
\author{Nathan A. McMahon}
\affiliation{ARC Centre for Engineered Quantum Systems, School of Mathematics and Physics, The University of Queensland, St Lucia, QLD, 4072, Australia}
\author{Gavin K. Brennen}
\affiliation{Center for Engineered Quantum Systems, Dept. of Physics and Astronomy, Macquarie University, 2109 New South Wales, Australia}
\author{Thomas M. Stace}
\affiliation{ARC Centre for Engineered Quantum Systems, School of Mathematics and Physics, The University of Queensland, St Lucia, QLD, 4072, Australia}
  \date{\today}
  
\begin{abstract}
%Holographic error correcting codes are finite rate codes that have shown promising properties. We develop an integer programming decoding algorithm for general stabiliser codes. The algorithm is also used to find the distance of codes. Using this decoder we find Pauli recovery rate for holographic codes, including a threshold against Pauli errors for the heptagon code.
%We develop an integer programming decoding algorithm for Pauli errors in general stabiliser codes. Using this we show numerical evidence that holographic codes have thresholds against Pauli errors. The heptagon code has a theshold of $4.8\%$ against dephasing errors and the zero rate HaPPY code has a Pauli threshold of $21.8\%$. Additionally we show that the distance of some holographic codes increase exponentially with number of physical qubits.
We develop a most likely error Pauli error decoding algorithm for stabiliser codes based on general purpose integer optimisation. Using this decoder we analyse the performance of holographic codes against Pauli errors and find numerical evidence for thresholds against Pauli errors for bulk qubits. We compare the performance of  holographic code families of various code rates and find phenomenological Pauli error thresholds ranging from $7\%$ to $16\%$, depending on the code rate.  Additionally we give numerical evidence that specific distance measures of the  codes we consider scales polynomially with number of physical qubits.
\end{abstract} 

\pacs{}

  \maketitle
 
%\section{Introduction} 
  



Recent interest in the overlap between quantum information and the bulk-boundary correspondence \cite{Harlow2016} has connected holography and error correction \cite{Latorre2015,Pastawski2015,Yoshida2013}. %In holography, $d$ bulk degrees of freedom are encoded in $d+1$ boundary degrees of freedom suggesting that there is substantial redundancy to the encoding. 
In holography, degrees of freedom (DOFs) in a $d+1$ dimensional bulk manifold are encoded in DOFs in a $d$ dimensional boundary manifold leaving substantial redundancy to the encoding. This redundancy makes holography a principle for developing quantum error correcting codes.



\begin{table}[t]
\begin{equation*}
\begin{array}{rlllllllll}
\textrm{index label:} & 1 & 2 & 3 & 4 & 5 & 6 & L & 7 \\ 
 \hline
 & X & X & \mathbb{I} & \mathbb{I} & \mathbb{I} & X & \mathbb{I} & X & \equiv S_1 \\ 
& \mathbb{I} & X & X & X & \mathbb{I} & \mathbb{I} & \mathbb{I} & X& \equiv S_2 \\ 
 & \mathbb{I} & \mathbb{I} & \mathbb{I} & X & X & X & \mathbb{I} & X& \equiv S_3 \\ 
 & Z & Z & \mathbb{I} & \mathbb{I} & \mathbb{I} & Z & \mathbb{I} & Z & \equiv S_4\\ 
 & \mathbb{I} & Z & Z & Z & \mathbb{I} & \mathbb{I} & \mathbb{I} & Z & \equiv S_5\\ 
& \mathbb{I} & \mathbb{I} & \mathbb{I} & Z & Z & Z & \mathbb{I} & Z & \equiv S_6\\
 & X & X & X & X & X & X & X & X & \equiv S_{\bar X}\\ 
& Z & Z & Z & Z & Z & Z & Z & Z & \equiv S_{\bar Z}
\end{array}
\end{equation*}
\caption{The ordered set of \emph{extended} stabilisers and logical operators that define the block-perfect Steane code tensor, $T_{S}^{j_1,...,j_L,j_7}$. The tensor is given by $T_{S}^{j_1,...,j_L,j_7}=\braket{j_1,...,j_L,j_7|T_S}$ where $\ket{T_S}$ is the $+1$ eigenstate of the eight commuting operators, $S_j$, above.}
\label{tab:SteaneTensor}
\end{table}


For practical quantum processing, error correction is essential \cite{Roffe2019,Preskill1998}. 
A good quantum error correcting code (QECC) ideally has four properties: a threshold against physical errors \cite{Barrett2010}; a finite ratio -- the code rate -- of the number of encoded to physical qubits \cite{Roffe2019}, low-weight  parity check operators \cite{Bohdanowicz2019}, and a fault-tolerant path to a universal gate set  \cite{Pastawski2015a}.  In this Letter, we study  code thresholds, rates and distances for a variety of holographic code families, to establish their performance against some of these metrics. 

\citet{Pastawski2015} (HaPPY) developed holographic quantum error correcting codes by tessellating tensor representations of the five qubit QECC \cite{Laflamme1996} on discretised negatively curved space. %The five qubit code was used because it is a \emph{perfect tensor} which is an extremely restricitive class that contains one known perfect code for qubits. 
Due to the proportional scaling between bulk and boundary volumes in a hyperbolic tiling, holographic error correcting codes can form finite rate error correcting codes. The rate of the code is tunable via modification of the tiling. HaPPY showed that the code with the maximum achievable rate did not have thresholds against erasures, however a version of the code with reduced rate was shown to have an erasure threshold which is comparable to that of  the surface code \cite{Stace2009, Stace2010, Barrett2010}.

The five qubit QECC was the first code used to generate holographic tilings because it has a \emph{perfect tensor} representation. %which is an extremely restrictive class that contains one known perfect code for qubits. 
This property is rare amongst known codes. More recently it has been shown that the perfect tensor condition can be relaxed to a  \emph{block perfect} condition \cite{Harris2018}, which coincides with the definition of planar perfect tangles \cite{Berger2018a}. This relaxation allows more choices for the seed codes used to generate the holographic tiling, extending the set of known holographic codes families to include a holographic code based on the Steane  code \cite{Steane1996} (called here the \emph{heptagon code} \cite{Harris2018}).  This was  also shown to have promising erasure thresholds \cite{Harris2018}. %which has been suggested as a %prerequisite of performance against other error channels 
%useful filter for identifying effective codes \cite{Delfosse2016,Delfosse2017}. 


CSS codes have a transversal  ${\textsc{CNOT}}$ gate; self-dual CSS codes also have transversal Hadamard gates \cite{Preskill1998a}. Additionally it is known how to construct any CSS code with graph states \cite{Bolt2016,Bolt2018} which is a powerful approach to measurement-based quantum computation. %Additionally there exists transversal clifford gate sets \cite{}.

Decoding erasures is numerically straightforward \cite{Harris2018}, but optimally decoding computational (e.g.\ Pauli) errors is a numerically hard problem in general \cite{Iyer2015} (though good decoders exist for  specific codes \cite{Sipser1996, Fowler2013,Liu2019}, such as the surface code \cite{Dennis2002,Delfosse2016,Darmawan2018,Delfosse2017} and the colour code \cite{Bombin2018,Kubica2019}). %, however decoding is still a hurdle for new codes including holographic codes.% to navigate.
Given the relative computational ease of decoding erasure errors, the performance of a new QECC against erasure has been proposed as a performance filter \cite{Delfosse2016,Darmawan2018}. The promising erasure thresholds for holographic codes therefore suggests further study is warranted. 

In this Letter we describe a general purpose decoding algorithm for stabiliser codes based on a global branch and bound integer optimisation \cite{gurobi}. We implement this decoder and numerically compute the performance of various holographic code families, including a new holographic code family based on a small surface code that we introduce here. %to show 
We provide numerical evidence of thresholds against Pauli errors for these holographic code families. Additionally we use related algorithms to find distances of the codes.






%\section{Holographic Codes}

\emph{Holographic code construction}: Holographic codes are seeded by an  $[[n,k,d]]$ QECC \cite{Gottesman1997}.  The seed QECC is described by a rank $(n+k)$ tensor, $T$, % with each tensor index dimension set by $q$. 
%Indices are grouped into qubits, which can be graphically represented as leg from a polygon \cite{Bridgeman2017}. 
%The tensor, $T$, can be written as a standard encoder 
which is the encoding map from logical to physical space $T: \mathcal{H}_{k} \mapsto \mathcal{H}_{n}$. %, with the conjugate $T^\dagger: \mathcal{H}_{q^n} \mapsto \mathcal{H}_{q^k}$ acting as a decoder. 
To be a valid code, $T$ must be an isometry, $T^\dagger T \propto \mathbb{I}$, which ensures perfect information recovery in the absence of noise.  We define the order-$(n+k)$ seed tensor %, $T_{S}^{j_1,...,j_{n+k}}$ is defined %by the Choi-Jamiolkowski isomorphism \cite{Jiang2013}. That is, 
as $T^{j_1,...,j_{n+k}}=\braket{j_1,...,j_{n+k}|T}$, where $\ket{T}$ is the $+1$ eigenstate of  all \emph{extended} stabilisers and logical operators, i.e.\ the extension of the operators to act on an $(n+k)$-qubit Hilbert space.%defined by the tensor product of the logical qubit and its respective code words. %in the logical state?

Conventionally, the tensor indices are arranged to form an encoding map, $T^{j_1,...,j_{n}\leftarrow j_{n+1},...j_{n+k}}:\mathcal{H}_{k} \mapsto \mathcal{H}_{n}$, from the $k$-dimensional logical Hilbert space to the $n$-dimensional physical Hilbert space.  Related codes can be defined with different index partitions, providing the encoding tensor remains an isometry. For example, if $T^{j_2,...,j_{n}\leftarrow j_1,j_{n+1},...j_{n+k}}$ is an isometry, then it is an encoding map for a $[[n-1,k+1,d^\prime]]$ code. %which can also be found via manipulation of the stabilisers \cite{Gottesman1997}.

%Multiple isometric tensors can be combined via tensor contraction to create composite codes, such as concatenated codes.%, providing the contracted tensor is still an isometry.

\emph{Perfect \& Block-Perfect Tensors}: Some classes of tensor that remain an isometry after a permutation of indices. We describe two such classes. Take a tensor with $m$ indices in an ordered set $J=\{j_1,j_2,...,j_{m}\}$. Partition $J$ into ordered subset $A$ and its complement $\overline{A}$, with some permutation $\Pi$ with respect to the reference index, i.e. $\{A|\overline{A}\}=\Pi[J]$. If under all permutations $\Pi$ the tensor remains an isometry then it is known as a \emph{perfect tensor} \cite{Pastawski2015}. %A weaker condition is restricting the permutations to cyclic shifts $\Pi = \sigma^p$, where $\sigma^p: j_i \rightarrow j_{i+p}$. 
If the tensor remains an isometry under all cyclic permutations \mbox{$\Pi = \sigma^p$}, where $\sigma^p: j_i \rightarrow j_{i+p}$, we call it \emph{block-perfect}.%this weaker condition it is defined as block perfect \cite{Harris2018}.

\begin{table}[t]
\begin{equation*}
 \begin{array}{rllllllllllllll}
\textrm{index label:}&1& &2& &3& &4& &L& &5\\
 \hline
 &X& &X& &I& &X& &\mathbb{I}& &\mathbb{I}&\equiv S_1& &\\
 &\mathbb{I}& &\mathbb{I}& &X& &X& &\mathbb{I}& &X&\equiv S_2& &\\
 &Z& &\mathbb{I}& &Z& &Z& &\mathbb{I}& &\mathbb{I}&\equiv S_3& &\\
 &\mathbb{I}& &Z& &\mathbb{I}& &Z& &\mathbb{I}& &Z&\equiv S_4& &\\ 
 &X& &\mathbb{I}& &X& &\mathbb{I}& &X& &\mathbb{I}&\equiv S_{\bar{X}}& &\\
 &\mathbb{I}& &\mathbb{I}& &Z& &\mathbb{I}& &Z& &Z&\equiv S_{\bar{Z}}& &
 \end{array}.
 \end{equation*}
\caption{The ordered set of stabilisers and logical operators that define the block-perfect surface code fragment tensor, $T_{\textrm{SCF}}^{j_1,...,j_L,j_5}=\braket{j_1,...,j_L,j_5|T_{\textrm{SCF}}}$ where $\ket{T_{\textrm{SCF}}}$ is the $+1$ eigenstate of $S_j$'s.}
\label{tab:SurfFragStabs}
\end{table}




As an example, the order-8 tensor associated with the Steane code \cite{Steane1996}, $T_{S}^{j_1,...,j_L,j_7}$, is block perfect \cite{Harris2018} with respect to the ordered set of extended operators defined in Table \ref{tab:SteaneTensor}.  The code family based on this seed code will be used in the following numerical results.



%\onecolumngrid

%\begin{figure}[t]
%	\centering
%	\subfloat[\label{fig:SurfFragment}]{%
%  		\includegraphics[clip,width=0.55\columnwidth]{SCF.pdf}%
%	}
%	
%	\subfloat[\label{fig:SinglePentagon}]{%
%  		\includegraphics[clip,width=0.45\columnwidth]{SinglePentagon.pdf}%
%	}\qquad	
%	\subfloat[\label{fig:SingleHexagon}]{%
%  		\includegraphics[clip,width=0.45\columnwidth]{SingleHexagon.pdf}%
%	}	
%	
%	\caption{(a) Lattice representing the $[[5,1,2]]$ surface code fragment (SCF) including stabilisers. Graphical representations of (b) a $[[5,1]]$ code tensor and (c) the $[[6,0]]$ state associated to a $[[5,1]]$ code.}
%\end{figure}
%\twocolumngrid

\begin{figure}
\centering
\includegraphics{PauliPaperSmallFigs.pdf}
\caption{(a) Lattice representing the $[[5,1,2]]$ surface code fragment (SCF) including stabilisers. Graphical representations of (b) a $[[5,1]]$ code tensor and (c) the $[[6,0]]$ state associated to a $[[5,1]]$ code. \label{fig:SingleHexagon} \label{fig:SinglePentagon} \label{fig:SurfFragment} }
\end{figure}

%Additionally we note here that the 
We also introduce a new holographic code based on the $[[5,1,2]]$ \emph{surface code fragment} (SCF), defined over 5 qubits, shown in \fig{fig:SurfFragment}a. The  SCF is a block-perfect, error-detecting CSS code. The order-6  SCF tensor, $T_{SCF}^{j_1,...,j_L,j_5}$ defined by the stabilisers in table \ref{tab:SurfFragStabs}, is an isometry for any block partition of indices from any cyclic permutation of $\{ 1,2,3,4,L,5 \}$.


%the tensor is also an isometry for any block partition of legs. 

%If under all permutations the tensor, or its conjugate, remains an isometry then the tensor is a \emph{perfect tensor} \cite{Pastawski2015}. A more general set is \emph{block perfect tensors}, where the tensor remains an isometry for all adjacent partitions in some cyclic ordering \cite{Harris2018}.


%Often a more intuitive picture can be formed by representing the code using a graphical tensor networks \cite{Bridgeman2017}. The tensor can be graphically represented 
Seed code tensors can be represented graphically as a polygon with a leg for each index of the tensor \cite{Bridgeman2017}. For a $[[n,k,d]]$ error correcting code, the standard graphical representation is an $n$-sided polygon, with a leg on each edge for the physical qubit indices and $k$ \emph{bulk} legs (dots) perpendicular to the face representing each logical qubit. For example \fig{fig:SinglePentagon}b is a representation of a $[[5,1]]$ code.

%Using the graphical language of tensor networks \cite{Bridgeman2017}, the tensor $T$ is described as an n-sided polygon with a leg from each edge representing the physical qubits and additional $k$ legs perpendicular to the face representing logical qubits. 

We conventionally interpret  polygons like \fig{fig:SurfFragment}b as a map from bulk to  planar indices. However, tensor indices can be partitioned into other subsets $A$ and $\overline{A}$: %One choice of partition is bulk and planar, but it is not unique. %In general the tensor can be recast as a map from any subset $A$ of legs to the complement $\overline{A}$. This is equivalent to rearranging the tensor indices. %As long as this map is an isometry then it describes some encoding, there are classes of tensors that remain an isometry for consistent permutation of indices.
if the tensor is an isometry for a particular choice of indices $A$, it describes an encoding map from $A$ to $\overline{A}$. For example, if the tensor in \fig{fig:SinglePentagon}b is block-perfect, then the tensor will be an isometry from  the indices $\{L,5\}$ to $\{1,2,3,4\}$, corresponding to  a $[[4,2]]$ code. 

%Multiple isometric seed tensors can be combined via index contraction to create composite codes, such as concatenated codes and holographic codes. 
%we are able to contract those legs with other tensors. This can be viewed as the outputs from one tensor are inputs into the second. If we tessellate tensors in such a way on a negatively curved surface we create a holographic code, which forms an isometry from all the bulk to the boundary qubits where we truncate our tessellation. 

To create holographic codes we tessellate seed codes, represented graphically as polygons-with-legs,  on a discretised 2D hyperbolic space, and contract tensor indices on linked edges. The tessellation is truncated at a particular \emph{radius}, $R$. %which is the minimum number of tensors from the centre to the boundary. 
For the heptagon code \cite{Harris2018} we tessellate heptagons which individually represent the Steane code \cite{Steane1996}; the version for $R=3$ is shown in \fig{fig:heptagontiling}a. If every polygon in the tesselation has an associated logical qubit, we call it a \emph{max-rate} holographic code.

%Alternately we can construct \emph{half-rate} codes, where the seed code polygons alternate between having bulk qubits and not.  these can form pentagon/hexagon codes \cite{Pastawski2015} as shown in \fig{fig:PentHex}. This pentagon/hexagon code can be seeded by pentagons/hexagons representing the surface code fragment from \fig{fig:SurfFragment} or the five qubit code \cite{Laflamme1996} as discussed by \citet{Pastawski2015}.

%Instead if we tessellate with pentagons representing the surface code fragment from \fig{fig:SurfFragment}, we get . Finally if the pentagon instead represent the five qubit code \cite{Laflamme1996} then we form a HaPPY code.

Additionally, we consider some tensor networks in which a subset of tiles in the tesselation do not have a logical input, as depicted in \fig{fig:SingleHexagon}c.  Such `blank' tiles do not add bulk logical legs to a network, but allow us to construct \emph{reduced-rate} codes by mixing such tiles amongst others that do have associated bulk indices. % by including blank polygons in a tessellation. %When alternating pentagons with hexagons we are approximately halving the rate of the code. 
%We can construct \emph{half-rate} codes, where the seed code polygons alternate between having bulk qubits and not. 
%Mixing tiles with and without a bulk index form reduced rate holographic codes. 
A particular realisation of this is the pentagon/hexagon code \cite{Pastawski2015}  shown in \fig{fig:PentHex}b, where blank tiles are interspersed in the tesselation.  We note that a given tiling built of order-$(n+k)$ tensors is consistent with any $[[n,k]]$ code.  For instance, the order-6 tensors shown in \fig{fig:PentHex}b  could represent either the $[[5,1,2]]$ surface code fragment from \fig{fig:SurfFragment}a or the $[[5,1,3]]$  five qubit code \cite{Laflamme1996} as introduced by \citet{Pastawski2015}.

%Combinations of blank hexagons and pentagons with a bulk index can form pentagon/hexagon codes \cite{Pastawski2015} as shown in \fig{fig:PentHex}. 

Lastly, we will also consider tilings in which only a single seed tensor, at the centre of the tiling, has a logical qubit associated to it, resulting in a  single-logical qubit code with \emph{zero-rate},  \cite{Pastawski2015}.%, where only the central tensor has bulk legs. 


% modify a code $[[n,k,d]]\rightarrow [[n-1,k+1,d^\prime]]$

%This forms an isometry from the bulk logical qubits to the boundary physical qubits. 

%The original work require the seed tensors to be perfect-tensors, that an isometry for any permutation of indices \citet{Pastawski2015}. Recently work has shown a more relaxed condition of block-perfect, an isomery for any adjacent partition of indices, is sufficent to generate a holograhic code \cite{Harris2018}. 

%Additionally \citet{Harris2018} showed that the Steane code met this condition and hence created the CSS Heptagon Code.


\begin{figure}
\includegraphics[clip,width=0.48\columnwidth]{HeptagonTilingLargeText1.pdf}\hfil
\includegraphics[clip,width=0.48\columnwidth]{PentHex1.pdf}
%\centering
%	\subfloat[\label{fig:heptagontiling}]{%
%  		\includegraphics[clip,width=0.45\columnwidth]{HeptagonTilingLargeText1.pdf}%
%	}
%	\subfloat[\label{fig:PentHex}]{%
%  		\includegraphics[clip,width=0.45\columnwidth]{PentHex1.pdf}%
%	}
\caption{Graphical tensor network representation of (a) the Heptagon code \cite{Harris2018} and (b) a reduced-rate Pentagon/Hexagon code. These describe maps from the red logical qubits in the bulk to the white boundary physical qubits. The seed tensor polygons in (b) could represent any $[[5,1]]$ and $[[6,0]]$ seed code tensors such as the SCF or 5-qubit code. }
\label{fig:heptagontiling}\label{fig:PentHex}
\end{figure}


%\textcolor{red}{
%\citet{Pastawski2015} construct holographic quantum error correcting codes based  on the \mbox{$[[n,k,d]]=[[5,1,3]]$} 5-qubit code \cite{Laflamme1996}. The 5-qubit code generates a rank $n+1=6$ \emph{seed tensor}, $T$, represented graphically as a pentagon in \fig{fig:pentagontensor}a. 
%%
%
%\citet{Pastawski2015} construct holographic quantum error correcting codes using  on the five qubit quantum error correcting code \cite{Laflamme1996}. Their \emph{pentagon code} is built on a tessellation of pentagons, with four meeting at each vertex (the $\{4,5\}$ Schl\"afli geometry). This is a surface with negative curvature, which can be visualised on a Poincar\'e disk. 
%
%
%The pentagon tensor network is constructed by tessellating a \emph{seed tensor} for the \mbox{$[[n,k,d]]=[[5,1,3]]$} five qubit code.
%
%Briefly, we represent tensors graphically as polygons, shown in \fig{fig:pentagontensor}. 
%The central vertex represents a logical input qubit, and the $n$ planar legs represent output qubits. The tensor specifies an isometry from logical input operators to output operators.} 

%\textcolor{red}{
%A larger tensor network is built from the seed tensor by tessellating it in the $\{4,n\}$ Schl\"afli geometry (i.e.\ with four polygons meeting at each vertex), forming a surface with negative curvature illustrated in \fig{fig:heptagontiling}c.  Neighbouring indices on adjacent tensors are contracted, which we represent graphically by connecting the corresponding planar legs \cite{Bridgeman2017}. %check other references
%%The tensor network for the pentagon code is constructed by tessellating the seed tensor, which generates a translationally invariant hyperbolic geometry. 
%The tessellation terminates at a certain radius $R$, which is given by the minimal number of edges from the boundary to the central \emph{bulk} logical qubit.  Input  vertices on each seed tensor in the bulk represent  logical bulk qubits; the uncontracted legs at the boundary terminate at  physical  qubits, denoted by hollow circles.
%}

%\textcolor{red}{
%The seed tensors in the pentagon holographic code are \emph{perfect tensors}, which we briefly review. For a rank $2m$  tensor, $T$, we may partition its indices into an ordered set $A$ and its ordered complement ${\bar A}$ such that \mbox{$\lvert A \rvert \leq \lvert {\bar A} \rvert=2m-\lvert A \rvert$}. We interpret $T$ as a linear map from the logical Hilbert space on the input indices in set $A$ to the image Hilbert space on the output indices in set ${\bar A}$, i.e.\
%%
%$
%T^{{\bar A} \leftarrow A} : \mathcal{H}_A \mapsto \mathcal{H}_{{\bar A}}.
%$}
%%

%\textcolor{red}{
%\citet{Pastawski2015} define $T$ to be a perfect tensor if it is an isometry for \emph{all} bipartitions of the indices  $\{A | {\bar A}\}$ with $\lvert A \rvert \leq \lvert {\bar A} \rvert$, i.e.\ $T$ satisfies
%%
%\begin{equation}
%\big(T^{{\bar A} \leftarrow A}\big)^\dagger T^{{\bar A} \leftarrow A} = \mathbb{I}_{\mathcal{H}_A}.
%\label{eq:perfectdef}
%\end{equation}
%This is a very restrictive constraint on $T$.}
%%

%\textcolor{red}{
%For later discussion, we note that we can express a given a bipartition of indices $\{A|{\bar A}\}$ as a permutation $\Pi$ with respect to some reference index ordering $\underline J=\{j_1,j_2,...,j_{2m}\}$, i.e.\ \mbox{$\{A|{\bar A}\}= \Pi[\underline J]$}. A perfect tensor is therefore an isometry for \emph{all} permutations $\Pi$. This formulation will help when we define the less restricted class of \emph{block perfect tensors}.
%}


%\textcolor{red}{
%Operators acting on the physical qubits on the boundary of the space are defined via \emph{operator pushing} \cite{Pastawski2015} from logical bulk qubits, through the tensor network, to the physical boundary qubits. For constructive purposes we assign a direction to each leg in the network, shown by arrows in \fig{fig:heptagontiling}c, indicating that an `output' index from one tensor contracts with an `input' index to an adjacent tensor. Each tensor in the network translates operators acting on input indices to operators acting on output indices, according to %Equivalent operators on spaces $A$ and ${\bar A}$, where $\lvert A\rvert \leq \lvert {\bar A} \rvert$, satisfy 
%\begin{equation}
%O^A=T^{A\leftarrow {\bar A}}O^{{\bar A}} \left(T^{A\leftarrow {\bar A}}\right)^\dagger.
%\label{eq:tensorpushing}
%\end{equation}
%For example, an identity operator on the logical input leg of a stabiliser code translates to any of the stabiliser group on the output legs.}

%To construct boundary operators, we push operators from the logical bulk qubits through the network to physical qubits on the boundary. 
%As a consequence,
%\textcolor{red}{
%We note that the bulk logical qubits near the boundary map, via operator pushing, to boundary operators that are localised on a small wedge of the physical boundary qubits, while logical operators for qubits deep within the bulk are highly delocalised over the boundary. A constructive method to generate a complete set of stabilisers is shown in appendix A.}


%\textcolor{red}{
%The perfect tensor property guarantees that tensor legs can be arbitrarily partitioned into inputs and outputs. While this was inspired by diffeomorphism invariance in the underlying AdS space \cite{Pastawski2015}, it is very restrictive.    %, which admits breaking and rejoining legs in arbitrary permutations throughout the network.
%%\citeauthor{Pastawski2015} show
%They show that the rank-6 seed tensor for the 5-qubit code is indeed a perfect tensor. 
%The resulting holographic code has finite rate $r=k/n=1/\sqrt{5}$ in the asymptotic limit. % (where $k$ and $n$ are the number of logical and physical qubits respectively).
% %substantive background
% %perfect tensors
% %difeomorphic invariance
% }
 

 %Intro
%Block Perfect Section
% \textcolor{red}{
%We now show %by example 
%that the perfect tensor constraint can be relaxed to a less restrictive class that still generates a holographic code.  This is motivated by the observation that in the hyperbolic tessellation in \cite{Pastawski2015}, input legs to a given seed tensor can be grouped into a contiguous block.  This new class includes the seven qubit Steane code \cite{Steane1996} tensor, which we use in a CSS holographic code based on a  tiling of heptagons.
%}




%\textcolor{red}{
%We define \emph{block perfect tensors} to be those that are isometries for all \emph{cyclic} permutations $\Pi=\sigma^p$ of $\underline J$, i.e.\ those for which  $\{A|{\bar A}\}=\sigma^p[\underline J]$, where $\sigma^p:j_i\mapsto j_{i+p}$ is a cyclic shift. This coincides with the description of perfect tangles developed independently \cite{Berger2018}. We believe this constraint on the seed tensor more closely corresponds to a discretisation of diffeomorphism invariance, though we do not comment on this further here. %Following the same arguement in \cite{Pastawski2015}, the heptagon holographic code approximates the lattice formulation of the RT formula. 
%}
%\begin{figure}
%\includegraphics[width=0.9\columnwidth]{Figures/HeptagonTilingNew.pdf}
%\caption{A tensor network representation of the $R=3$ Heptagon Code. Here the eight legged tensors represent the Steane code, where the red logical leg is perpendicular to the page. The white dots round the outside are the boundary code qubits. The numbering is an example of the leg ordering required to produce an isometry from bulk to boundary. The background is a Poincar\'e disk demonstrating the tiling.}
%\label{fig:heptagontiling}
%\end{figure}
 


 
% Block Perfect Tensors  

%formalise block perfect definition
%cyclic permutation label??
%T_{1,2..}= ...


% Steane Code, CSS, construction


%\textcolor{red}{
%\emph{Steane Tensor}: We exemplify this relaxation of perfection by showing that the rank-8 Steane tensor, $T^{j_1,...,j_L,j_7}_{\mathrm{Steane}}$, which is generated from the  Steane code, is block perfect, but not perfect.  This tensor is defined through the unique simultaneous $+1$ eigenstate, $\ket{T_{\mathrm{Steane}}}$, of the 8 stabilisers
%turn into array
%\begin{equation}
%\begin{aligned}
%&\hat{\mathbb{I}}_L \rightarrow \hat{X}_1 \hat{X}_2 \hat{\mathbb{I}}_3 \hat{\mathbb{I}}_4 \hat{\mathbb{I}}_5 \hat{X}_6 \hat{X}_7 = S_1 \\
%&\hat{\mathbb{I}}_L \rightarrow \hat{\mathbb{I}}_1 \hat{X}_2 \hat{X}_3 \hat{X}_4 \hat{\mathbb{I}}_5 \hat{\mathbb{I}}_6 \hat{X}_7 =S_2\\
%&\hat{\mathbb{I}}_L \rightarrow \hat{\mathbb{I}}_1 \hat{\mathbb{I}}_2 \hat{\mathbb{I}}_3 \hat{X}_4\hat{X}_5\hat{X}_6\hat{X}_7 =S_3\\
%& \hat{\mathbb{I}}_L \rightarrow \hat{Z}_1 \hat{Z}_2 \hat{\mathbb{I}}_3 \hat{\mathbb{I}}_4 \hat{\mathbb{I}}_5 \hat{Z}_6 \hat{Z}_7 =S_4\\
%& \hat{\mathbb{I}}_L \rightarrow \hat{\mathbb{I}}_1 \hat{Z}_2\hat{Z}_3 \hat{Z}_4 \hat{\mathbb{I}}_5 \hat{\mathbb{I}}_6 \hat{Z}_7 =S_5\\
%& \hat{\mathbb{I}}_L \rightarrow \hat{\mathbb{I}}_1 \hat{\mathbb{I}}_2 \hat{\mathbb{I}}_3 \hat{Z}_4\hat{Z}_5\hat{Z}_6\hat{Z}_7 =S_6\\
%& \hat{X}_L \rightarrow \hat{X}_1 \hat{X}_2 \hat{X}_3 \hat{X}_4 \hat{X}_5 \hat{X}_6 \hat{X}_7 =\overline{X}\\
%& \hat{Z}_L \rightarrow \hat{Z}_1 \hat{Z}_2 \hat{Z}_3 \hat{Z}_4 \hat{Z}_5 \hat{Z}_6 \hat{Z}_7 = \overline{Z}.
%\end{aligned}
%\end{equation}
%\begin{equation}
%\begin{array}{rlllllllll}
%\textrm{index label:} & 1 & 2 & 3 & 4 & 5 & 6 & L & 7 \\ 
% \hline
% & X & X & \mathbb{I} & \mathbb{I} & \mathbb{I} & X & \mathbb{I} & X & \equiv S_1 \\ 
%& \mathbb{I} & X & X & X & \mathbb{I} & \mathbb{I} & \mathbb{I} & X& \equiv S_2 \\ 
% & \mathbb{I} & \mathbb{I} & \mathbb{I} & X & X & X & \mathbb{I} & X& \equiv S_3 \\ 
% & Z & Z & \mathbb{I} & \mathbb{I} & \mathbb{I} & Z & \mathbb{I} & Z & \equiv S_4\\ 
% & \mathbb{I} & Z & Z & Z & \mathbb{I} & \mathbb{I} & \mathbb{I} & Z & \equiv S_5\\ 
%& \mathbb{I} & \mathbb{I} & \mathbb{I} & Z & Z & Z & \mathbb{I} & Z & \equiv S_6\\
% & X & X & X & X & X & X & X & X & \equiv S_{\bar X}\\ 
%& Z & Z & Z & Z & Z & Z & Z & Z & \equiv S_{\bar Z}
%\end{array},
%\label{eq:SteaneTensor}
%\end{equation}
%via the Choi-Jamio\l kowski isomorphism \cite{Jiang2013}.
%That is, $T^{j_1,...,j_L,j_7}_{\mathrm{Steane}}=\langle j_1,...,j_L,j_7\ket{T_{\mathrm{Steane}}}$ where  $\ket{T_{\mathrm{Steane}}}$ satisfies  $S_\alpha\ket{T_{\mathrm{Steane}}}=\ket{T_{\mathrm{Steane}}}$ for all $\alpha$. The index labels in \eqn{eq:SteaneTensor} are consistent with the ordering shown in figure \fig{fig:heptagontensor}b. With respect to this index label ordering, we have exhaustively checked that $T_{\mathrm{Steane}}$ is block perfect.
%}
%We define the code generating tensor as:
%%
%\begin{equation}
%\begin{aligned}
%G_{Steane}=&\left(\frac{\mathbb{I}^{\otimes 8}+\mathbb{I}_L\otimes S_1}{2}\right)\left(\frac{\mathbb{I}^{\otimes 8}+\mathbb{I}_L\otimes S_2}{2}\right) ... \\
%& \times \left(\frac{\mathbb{I}^{\otimes 8}+X_L\otimes \overline{X}}{2}\right)\left(\frac{\mathbb{I}^{\otimes 8}+Z_L\otimes \overline{Z}}{2}\right),
%\end{aligned}
%\end{equation}
%which has a unique $+1$ eigenstate $G_{Steane}\ket{T_{Steane}}=+\ket{T_{Steane}}$, we define  $\bra{1}\ket{2}$
%This is the same tensor as the code tensor, up to a reorganisation of legs.

%\textcolor{red}{
%It is straightforward to see that $T_{\mathrm{Steane}}$ is \emph{not} a perfect tensor, by considering the non-contiguous partition of indices $A=\{3,4,5,L\}$ and ${\bar A}=\{1,2,6,7\}$. If $T_{\mathrm{Steane}}$ were perfect, then $T^{A\leftarrow {\bar A}}$ would be unitary. Then according to \eqn{eq:tensorpushing}, \mbox{$T^{A\leftarrow {\bar A}}X^{\otimes A} \big(T^{A\leftarrow {\bar A}}\big)^\dagger\neq\mathbb{I}^{\otimes {\bar A}}$}. However according to $S_1$, and the Choi-Jamio\l kowski isomorphism
%\mbox{$T^{A\leftarrow {\bar A}}X^{\otimes A} \big(T^{A\leftarrow {\bar A}}\big)^\dagger = \mathbb{I}^{\otimes {\bar A}}$}, implying that for this partition, $T^{A\leftarrow {\bar A}}$ is not a unitary map.  Hence $T_{\mathrm{Steane}}$ is not perfect.
%}

%\textcolor{red}{
%\emph{Heptagon Holographic Code}: As with the pentagon code, the heptagon code is built on a 2D tiling with negative curvature. This is a tessellation of heptagons, with four heptagons meeting at each vertex (the $\{4,7\}$ Schl\"afli geometry), as shown in \fig{fig:heptagontiling}c.
%}
%\textcolor{red}{
%The hyperbolic tiling of the heptagon code requires a consistent assignment of  index contractions between adjacent tensors. \fig{fig:heptagontiling}c shows one such assignment for a subset of the tiles. This ensures that every seed tensor indeed acts as an isometry from inputs to outputs, so that the entire network is an isometry from bulk inputs to boundary outputs. 
%}
%describe code tensor: unique +1 eigen state of code projector
%

%tensor injection/pushing

%tensor action in heisenberg/clifford picture picture cite gottesman 97/ rausendorf 2005





%As we require an isometry from the bulk to the boundary, we must ensure the positioning of the legs is such that the inputs from the previous layer are adjacent legs to the planar logical. For the ordering above this means for the tensors with one leg contracted with the previous layer it must be either 6 or 7, where there are two contracted it must be a choice of two that forms an adjacent block with the logical in planar form. One example of a sufficient leg ordering is shown in \fig{HeptagonTiling}.

% New tessalation

%\textcolor{red}{
%Because the seed code is a self-dual CSS code, it is clear that pushing $X$-like tensors will lead to $X$-like holographic stabilisers, and similarly for the $Z$-like stabilisers. This means the heptagon holographic code is a self-dual CSS code. Similarly to the pentagon code, the heptagon code is a finite rate code, with asymptotic rate  $r=1/\sqrt{21}$.
%}
%\textcolor{red}{
%Block-perfect tensors in a hyperbolic tiling generate a holographic code according to the definition in \citeauthor{Pastawski2015}, based on the existence of a greedy algorithm.  
%%The greedy algorithm  constructs a \emph{recoverability region}, $\mathcal{R}$, of bulk logical data by recursively adding bulk tensors, $T$ to $\mathcal{R}$ according to the local update rules: (1) boundary qubits are `recoverable' if they are not erased; and (2) given some set, ${\bar A}$, of tensor indices for $T$ that are `recoverable', then if there is an isometry from $A$ to ${\bar A}$ (note $\lvert A \rvert \leq \lvert {\bar A} \rvert$), we add $T$ to $\mathcal{R}$. The fixed point of these rules defines $\mathcal{R}$.   %   , which works by collecting bulk tensors into a \emph{recoverability region} if there are three legs or more contracted with the recoverability region already.
%%As with the pentagon code, the block-perfect  tensor construction admits a greedy algorithm, and therefore, according to \cite{Pastawski2015} the RT formula holds, $S_{\partial \mathcal{R}}\propto \textrm{Area}(\mathcal{R})$, for contiguous boundary regions $\partial \mathcal{R}$. 
%The greedy algorithm constructs a recoverability region, $\mathcal{R}$, of bulk logical data by recursively adding bulk tensors, $T$ to $\mathcal{R}$ according to the local update rules: (1) boundary qubits are `recoverable'�� if they are not erased; and (2) given some set, ${\bar A}$, of tensor indices for $T$ that are recoverable��, then if there is an isometry from $A$ to ${\bar A}$  (with $\lvert A \rvert \leq \lvert {\bar A} \rvert$), then we add $T$ to $\mathcal{R}$. The fixed point of these rules defines $\mathcal{R}$. For holographic codes built from perfect tensors, the tensor indices in ${\bar A}$ can be arbitrary, whereas for  block perfect tensors they must be in contiguous order. Starting from a contiguous region $B$ on the boundary, the region $\mathcal{R}$ produced by this algorithm has an inner boundary that approximates, to within a small constant, the discrete bulk geodesic $\gamma_B$ connecting the end points of B. As shown in \cite{Pastawski2015} this implies an RT formula of $S_B \propto \lvert\gamma_B\rvert$.
%}

%Here one absorbs a tensor into a growing bulk+boundary region P if the tensor defines an isometry from inputs outside P to outputs in P. Starting from P=A, the process stops when no further tensors can be absorbed leaving a final bulk + boundary region P. The bonds connecting P to the rest of the bulk defines gamma*_A. For connected regions, the performance of the greedy algorithm works essentially the same for block perfect as for perfect tensors since the flow of isometries can be arranged in sequentially ordered sets of indices.

%\textcolor{red}{
%\emph{Erasure decoders}: Having defined the heptagon holographic code we are interested in the resilience of the code to errors. \citet{Delfosse2016} propose using the robustness of a code to erasure errors as a proxy for performance of the code under more general error channels. As such, we now describe an erasure decoder for this code, with which to quantify the code performance.
%}

%\textcolor{red}{
%Loss errors are heralded, so that we know where they have occurred. This enables us to use the error pattern as part of the error decoding algorithm, making an exact decoder computationally feasible. %The greedy algorithm created by \citeauthor{Pastawski2015}, described above, is not optimal for erasure errors.%\citeauthor{Pastawski2015} created a greedy heuristic decoder to reconstruct the bulk operators after erasure. This algorithm uses local update rules (relative to the tensor geometry) to determine whether a given bulk logical qubit is recoverable, but is not optimal.
%}

%\section{Pauli Decoder}
\emph{Pauli Decoder}: In contrast to erasure decoders, optimally correcting Pauli errors for general stabiliser codes is \#P-complete  \cite{Iyer2015}. %For some specific codes, the code properties allow simplification of this problem \cite{Sipser1996, Fowler2013,Liu2019}. %, and some machine learning techniques have shown speed up \cite{Tan2010, }. 
Here we use general purpose integer optimisation software to perform most likely error (MLE) correction for general stabiliser codes, albeit with a high computational cost. This is useful for evaluating new QECCs, even if it is impractical for real-time experimental implementations. 
The algorithm can be applied to any stabiliser code, with suitable adjustments from the CSS variant described here, which we use to compute numerical thresholds for a Pauli error channel for the heptagon code, the SCF code and the  HaPPY code \cite{Pastawski2015}.

%\emph{Recovery Algorithm}:
%
%  \section{Logical Support Vector Notation}
%Stabiliser codes can be described in the language of binary vector spaces . For this 
We represent operators as binary symplectic vectors (BSV) \cite{Calderbank1997, Gottesman1997,Dehaene2003} for $X$ and $Z$ components defined for $n$-qubit operator $\hat{A}$ as%. For CSS codes the $X$ and $Z$ like BSVs, $\underline{s}_{Xj}$ and $\underline{s}_{Zj}$, are defined by
%
%\begin{equation}
%\mathcal{S}_{Xj}=\hat{X}^{\otimes \underline{s}_{Xj}} \qquad
%\mathcal{S}_{Zj}=\hat{Z}^{\otimes \underline{s}_{Zj}}.
%\end{equation} 
\begin{equation}
\hat{A}={\otimes}_j \hat{X}^{(\underline{a}_X)_j}\hat{Z}^{(\underline{a}_Z)_j}\equiv\hat{X}^{\otimes \underline{a}_X}\hat{Z}^{\otimes \underline{a}_Z}
\end{equation}
where  $\underline{a}_X, \underline{a}_Z \in \mathbb{Z}_2^n$. % are binary vectors of length $n$. %If $a_{Xi}=1$ while $a_{Zi}=0$ that indicates $\hat{A}$ has an $\hat{X}$ operator in the i-th qubit, while in the reverse indicates a $\hat{Z}$. If both are $0$ or $1$ that indicate as either a trivial operation or $\hat{Y}$ operator respectively.
For CSS codes, either $\underline{a}_X$ or $\underline{a}_Z$ will be zero for a given stabiliser or logical operator. Further, for a self-dual CSS code such as the heptagon code %the non-zero vectors can be written in a form such that 
for any $X$ type stabiliser with $(\underline{a}_X,\underline{a}_Z) = (u,0)$ there is a corresponding $Z$ type stabiliser with $(\underline{a}_X,\underline{a}_Z) = (0,u)$.

% Similarly we can define logical operator BSV. 

To perform decoding we assume
%When modelling error correction in self-dual CSS codes we consider 
$X$ and $Z$ type errors are I.I.D, similarly to the minimum weight perfect matching decoder for surface codes. However for our simulations we simulate a depolarising error channel, while decoding with the previous assumption. %separately. By symmetry any results will be identical for $X$ and $Z$ type errors. 
For clarity we %drop explicit Pauli labels and
 describe a decoder for a self-dual $[[n,k]]$ CSS QECC subject to $Z$ errors;  $X$ errors are treated in the same way. %Here we describe a decoder for a CSS code with $Z$ errors, hence will drop reference to $X$ or $Z$ from here on. 
We consider a generic dephasing error given by
% \begin{equation}
% \hat{\mathcal{E}}=\hat{Z}^{\otimes \underline{\varepsilon}},
% \end{equation}
\mbox{$
 \hat{\mathcal{E}}=\hat{Z}^{\otimes \underline{\varepsilon}}
$}. %is an $n$-dimensional BSV.
%and then use the stabilisers to calculate the syndrome. 
We define the parity check matrix $\underline{\underline{S}}$, where each stabiliser BSV, $\underline{s}_{j}$, forms a row of the matrix, so that $\underline{\underline{S}}$ is an $\frac{n-k}{2}\times n$ dimensional matrix.  The error syndrome is then given by \mbox{ $\underline{y}=\underline{\underline{S}} \cdot \underline{\varepsilon}$}.
 
%The length $\frac{n-k}{2}$ syndrome vector $\underline y$ can be found by multiplying the parity check matrix by the error BSV \mbox{ $\underline{y}=\underline{\underline{S}} \cdot \underline{\varepsilon}$}.
%\begin{equation}
% %\underline{y}_{\frac{n-k}{2}}=\underline{\underline{S}}_{\frac{n-k}{2}\times n} \cdot \underline{\varepsilon}_n.
% \underline{y}=\underline{\underline{S}} \cdot \underline{\varepsilon}.
%\end{equation} 
 
%A common decoding approach is to find a maximum likelihood error string that is consistent with the syndrome $y$. For an IID error model, the maximum likelihood error is the lowest weight error operator that is consistent with the syndrome. 

%We use a maximum likelihood decoder to find a correction. For an IID error model, the maximum likelihood error is the lowest weight operator that is consistent with the syndrome. 
 
 %Our decoder finds maximum likelihood errors, ie. we find a lowest weight error that would produce the known syndrome. For an IID error model this is a maximum likelihood error consistent with the syndrome. 
%\section{Inverse Syndrome Former} 
 
%From here we will drop reference to X or Z type as this all applies equally to both in CSS codes.

From the syndrome we employ an inverse syndrome former (ISF) to find a correction that returns us to the code space. The %$n\times\frac{n-k}{2}$-dimensional
 ISF matrix $\underline{\underline{F}}$ is the pseudoinverse (mod 2) of the parity check matrix, satisfying
 %We create the inverse syndrome former (ISF) support matrix, $\underline{\underline{F}}$, which is the pseudo-inverse of the stabiliser matrix, that is it satisfies 
 %\begin{equation}
 %\underline{\underline{F}}^T_{\frac{n-k}{2}\times n} \cdot \underline{\underline{S}}^T_{n \times \frac{n-k}{2}}=\mathbb{I}_{\frac{n-k}{2} \times \frac{n-k}{2}}.
\mbox{ $\underline{\underline{F}}^T \cdot \underline{\underline{S}}^T=\mathbb{I}
%_{\frac{n-k}{2} \times \frac{n-k}{2}}
$}.
% \end{equation}
That is, each column of the ISF defines an operator that anticommutes with only the corresponding stabiliser. It is not always possible to find an ISF in this way, for example in the toric code each error anticommutes with two stabilisers.
%The ISF can be formed by having each row, $j$ a BSV representing an error that anti-commutes with only the $j$th stabiliser. 
%As the identity is in the smaller dimension, number of stabilisers, the ISF is non-unique. It can be constructed using the procedure that the j-th row of the ISF with break only the stabiliser of the j-th column of the stabiliser matrix.
We use $\underline{\underline{F}}$, along with the syndrome to find a \emph{pure error} BSV, $\underline{e}=\underline{\underline{F}} \, \underline{y}$, that satisfies the syndrome, $\underline{y}=\underline{\underline{S}} \cdot \underline{\varepsilon} = \underline{\underline{S}} \cdot \underline{e}$.

%\begin{equation}
%\underline{e}=\underline{\underline{F}} \, \underline{y}.
%\end{equation}
%which, if applied to the state with errors, would return us to a random code word as the syndrome is degenerate.

%\section{Optimisation}

  \begin{figure*}[t]
  \includegraphics[clip,width=0.32\columnwidth]{HeptagonDepolarisingInset.pdf}
  \includegraphics[clip,width=0.32\columnwidth]{ElliotPentHexDepolarising.pdf}
  \includegraphics[clip,width=0.32\columnwidth]{HappyZeroRateDepolarising.pdf}
	
	\caption{Failure probability of the central logical qubit in the a) Max-rate Heptagon Code, b) Reduced-rate SCF Code and c) Zero-rate HaPPY code, in the presence of a depolarising channel.  The inset to fig (a) shows the same data on log-scale to show the performance well-below threshold. Note the error region around the lines are not significantly wider than the lines themselves. The heptagon code raw data with error bars in shown in figure \ref{fig:ErrorGraphs} in the appendix. \label{fig:PauliGraphs} }
\end{figure*}

%Since logical operators and stabilisers commute with all the stabilisers, if we multiply any stabiliser or logical operator with a pure error $\hat{E}=\hat{Z}^{\otimes \underline{e}}$, it will still satisfy the syndrome. Further, t
The complete set of errors that satisfy the syndrome is generated by the product of all combinations of stabilisers and logical operators with $\hat{E}=\hat{Z}^{\otimes \underline{e}}$.  All such errors have BSV of the form % so that any error can be expressed as % generic error that satisfies the syndrome is given by
\begin{equation}
\underline{e}^\prime=\underline{e}+{\sum}_{\ell=1}^{\frac{n-k}{2}}\lambda_\ell \underline{s}_\ell + {\sum}_{m=1}^{k}\mu_m \underline{l}_m,
\label{eq:correction_normal}
\end{equation}
where $\lambda_\ell, \mu_m \in \mathbb{Z}_2$ and  $\underline{l}_m$ is a logical operator BSV. %  will also generate the same syndrome for any $\lambda$ and $\mu$.
%for a self-dual code with $n-k$ stabiliser generators and $k$ logical qubits. 

 For an IID error model, a MLE decoder  minimises the Hamming weight of $e^\prime$ over $\lambda$ and $\mu$, to find a most likely correction chain
%\begin{equation}
%\underline{c}=\arg\min\limits_{\lambda, \mu \in \mathbb{Z}_2} \textrm{wt}\left[\underline{e}^\prime\right],
%\label{eq:maxliklihoodcorr}
%\end{equation}
$\underline{c}=\arg\min\limits_{\lambda, \mu \in \mathbb{Z}_2} \textrm{wt}[\underline{e}^\prime]$, 
where $\textrm{wt}$ is the Hamming weight of the vector.  Minimising $\textrm{wt}[\underline{e}^\prime]$ over $\lambda$ and $\mu$  is an integer optimisation problem. %We use the integer optimiser recovery algorithm detailed above to find a maximum likelihood correction using the Gurobi optimisation package 
We implement this optimisation problem using the Gurobi optimisation package \cite{gurobi}. For the examples shown here Gurobi performs global optimisation on the problem.




%\section{Monte-Carlo Simulations}
\emph{Performance Simulations}: We analyse the performance of the  codes against Pauli errors using Monte-Carlo simulation of an IID depolarising error model, with error rate $p$.  %We generate error chains numerically, from which we compute the syndrome, which we pass to the integer optimising decoder.  
We generate IID patterns of Pauli errors for a fixed number of errors $a=\mathrm{wt}(\underline{\varepsilon})$, from which we compute the syndrome, which we pass to the integer optimising decoder. To decide if the decoder has been successful, we calculate the net error after decoding, which is the product of the original error and the correction, $\underline{\varepsilon}+\underline{c}$. The decoder is successful if the net error acts trivially on the logical code space.

We iterate over all $0\leq a\leq n$ to estimate the recovery probability, $P_{\mathrm{failure}}(a,n)$, and use the binomial formula
\begin{equation}
p_{\textrm{failure}}(p, n)=\sum_a {n\choose a} p^a (1-p)^{n-a} P_{\mathrm{failure}}(a,n),
\label{eq:binomial}
\end{equation}
to calculate the recovery rate for different error rates $p$.

Sampling over many error instances, and different error rates allows us to estimate thresholds in the usual way \cite{Barrett2010}.

We run the decoder for a variety of different tilings and codes.  These include: Heptagon tiling  based on the Steane QECC,  a pentagon tiling  code based on the $[[5,1,3]]$ qubit QECC (i.e.\ the HaPPY code), and a different pentagon tiling based on a $[[5,1,2]]$ surface error-detecting code.  For these broad groups, we encode different numbers of logical qubits, ranging from a single logical qubit at the centre of the tiling which asymptotically has zero rate, to maximum-rate encodings with as many logical qubits as possible.



Further, logical qubits in a given code are not homogeneous: logical qubits encoded near the boundary are protected by fewer stabilisers compared to logical qubits encoded closer to the centre of the tesselation.  As such, here we report threshold figures for the performance of the central logical qubit only.



In Fig \ref{fig:PauliGraphs}a we show the failure probability of the central logical qubit for the max-rate Heptagon code ($r\approx 0.22$) against IID Pauli errors
. With this decoder we see numerical evidence of a threshold near $p\approx7.0\%$ for the central logical qubit.

This threshold is comparable with the surface code which has a threshold of $15.5\%$ for the same noise model with a minimum weight perfect matching decoder \cite{Dennis2002,Wang2010}, albeit with  zero rate. %check cite

 
We also show the performance of the code  below threshold in the inset of Fig \ref{fig:PauliGraphs}a, which shows that the logical failure rate, $p_{\textrm{failure}}$, decreases exponentially with $p_{\textrm{depolarising}}$. 



In Fig \ref{fig:PauliGraphs}b we show the performance of the reduced-rate $[[5,1,2]]$ holographic code. Here we see a pronounced difference between odd radii, where the outer tensors have bulk logical qubits, and even. These are characterised by very different codes rates %(\mbox{$r_{\textrm{odd}}=( 3\sqrt{6}+4)/38\approx0.3$} and \mbox{$r_{\textrm{even}}=(3\sqrt{6}-4)/38\approx0.09$}.)
(\mbox{$r_{\textrm{odd}}\approx0.3$} and \mbox{$r_{\textrm{even}}\approx0.09$}), and we find thresholds at $p_\textrm{odd}\approx7.1\%$ and $p_\textrm{even}\approx8.2\%$ respectively.%There appears to be a threshold for odd radii at $p\approx7.1\%$ and a threshold for even radii at $p\approx8.2\%$. There is a similar distinction in asymptotic rates for the reduced rate code, the rates are $r_{\textrm{even}}=\frac{1}{38}(-4 + 3\sqrt{6})\approx0.09$ and $r_{\textrm{odd}}=\frac{1}{38}(4 + 3\sqrt{6})\approx0.3$.%where the higher rate is for the odd radii.} 

Additionally we consider the performance of the zero-rate HaPPY code, shown in Fig \ref{fig:PauliGraphs}c. We see evidence of a  threshold here at $16.3\%$. We note that this was the only non-CSS code we analysed with the decoder.  Even though the code has the same tiling as the  SCF (which is CSS),  the decoder run-time and memory consumption was vastly greater than the decoder applied to CSS codes.  As a result, we were only able to estimate the performance of the HaPPY code up to $R=3$, making this threshold estimate merely provisional.


% The Supplementary Material shows performance curves for a variety of codes.  A few have notable characteristics.  For example, we find numerical evidence of a threshold for the max-rate Heptagon code ($r\approx 0.22$)  at around $p\approx7.0\%$. 
% %, so in the asymptotic limit of large code size, if the probability of dephasing errors is less than $5\%$ we can always correct them.
% This threshold is comparable with the surface code which has a threshold of $15.5\%$ for the same noise model with a minimum weight perfect matching decoder \cite{Wang2010}, but with zero rate. %check cite

\begin{figure}
\includegraphics[width=0.9\textwidth]{ThresholdRatePlot.pdf}
\caption{A comparison of asymptotic rate and numerically estimated threshold against depolarising errors. of holographic codes seeded with the Heptagon (`Steane') code, the $[[5,1,3]]$  SCF code, and the five qubit $[[5,1,3]]$ code (HaPPY). There is an inverse relationship between threshold and rate.}
\label{fig:ThresholdRatePlot}
\end{figure}

%In the reduced-rate SCF holographic code (whose tiling is shown in Fig.\ \ref{fig:PentHex}b), we find a pronounced difference between odd radii, where the outer tensors have bulk logical qubits, and even radii.  These are characterised by very different codes rates %(\mbox{$r_{\textrm{odd}}=( 3\sqrt{6}+4)/38\approx0.3$} and \mbox{$r_{\textrm{even}}=(3\sqrt{6}-4)/38\approx0.09$}.)
%(\mbox{$r_{\textrm{odd}}\approx0.3$} and \mbox{$r_{\textrm{even}}\approx0.09$}), and we find thresholds at $p_\textrm{odd}\approx7.1\%$ and $p_\textrm{even}\approx8.2\%$ respectively (see Supplementary Material). %There is a similar distinction in asymptotic rates for the reduced rate code, the rates are \mbox{$r_{\textrm{even}}=(3\sqrt{6}-4)/38\approx0.09$} and \mbox{$r_{\textrm{odd}}=( 3\sqrt{6}+4)/38\approx0.3$}.%where the higher rate is for the odd radii. 

%Lastly, for the zero-rate HaPPY code, we see some evidence of a  threshold  at  $p\approx16\%$ (see Supplementary Material).  We note that this was the only non-CSS code we analysed with the decoder.  Even though the code has the same tiling as the  SCF (which is CSS),  the decoder run-time and memory consumption was vastly greater than the decoder applied to CSS codes.  As a result, we were only able to estimate the performance of the HaPPY code up to $R=3$, making this threshold estimate merely provisional.

Fig.\ \ref{fig:ThresholdRatePlot} summarises a larger set of numerical simulations, plotting the rate and threshold for a variety of different holographic codes.  We see the expected tradeoff between rate and threshold quite clearly.  Of the codes we have analysed, none dominates the others: increasing rate never increases the threshold, although there are regions where the tradeoff frontier is notably flat.


%\section{Distance}
\emph{Distance}: The decoder also provides a way to find the distance of a code, using the integer optimiser to find the minimum weight logical operator.  
Strictly all maximum rate holographic codes have a fixed distance equal to the distance of the seed code:  this is the distance of the logical qubits closest to the boundary. 
However bulk qubits further from the boundary are better protected than this distance suggests.  A fuller picture is formed by considering the distance of each logical qubit separately. 



We define two distance measures  for each  logical qubit. Firstly the logical \emph{bit distance} is the lowest weight logical operator associated to logical qubit $i$ that acts trivially on all other logical qubits, ie.
\begin{equation}
d_i^{(B)}= \min\limits_{\lambda}\textrm{wt}\Big[\underline{l_i}+{\sum}_{j=1}^{J}\lambda_j \underline{s_j}\Big].\nonumber
\end{equation}
Secondly the \emph{word distance} is the minimum weight logical operator that has support on logical qubit $i$, but may act non-trivially on other logical qubits. This distance is equivalent to the distance measure by \citet*{Pastawski2017a}. This is calculated using
\begin{equation}
d_i^{(W)}= \min\limits_{\lambda, \mu} \textrm{wt}\Big[\underline{l_i}+{\sum}_{j=1}^{J}\lambda_j \underline{s_j} + {\sum}_{k\neq i}^{}\mu_k \underline{l_k}\Big].\nonumber
\end{equation}
The word distance counts the shortest weight error that would go undetected but would corrupt the data, while the generally larger bit distance counts how large a logical operator need be to act on an isolated logical qubit, useful e.g. to work out fault tolerant constructions thereof.



Both of these distances can be found using the same integer optimisation package used for decoding.  For different code radii in a given code family we compute the code distance, $d$, and fit a power-law as a function of the number of physical qubits.
%(see Supplementary Material for the example of the Heptagon code).   Table \ref{tab:distacetable} summarises these results for $d_{\textrm{central}}^{(B,W)}$ for the central logical qubit.  
 \fig{fig:HeptagonDistance} shows the heptagon code distances (for the central logical qubit) against the number of physical qubits. We see numerical evidence of a power law scaling of distance with the number of physical qubits for both measures.  Similar results are found for other code families.   Table \ref{tab:distacetable} shows the results of numerically found code distances for the other codes studied here, along with the results of power law fits to the numerical results.




We also note that while the numerics here are for the central logical qubit, the important parameter is the bulk qubit distance from the boundary. We say a bulk qubit is positioned at radius $r$, which is the number of tensors between the bulk qubit and the centre. For example, the radius of the central qubit $r=0$ and boundary bulk qubits $r=R-1$. For a given seed tensor and tessellation, the bit distance $d^{(B)}_{R-r}$ is constant for a given value $R-r$, this is also true for word distance.
\begin{figure}[t]
\includegraphics[width=0.95\textwidth]{HeptagonDistance.pdf}
\caption{The distance of the central logical qubit for the heptagon code at different radii, both the bit and word distance scale exponentially with the number of physical qubits. The fit lines are $d^{(W)}=n^{0.37}$ and $d^{(B)}=n^{0.54}$.}
\label{fig:HeptagonDistance}
\end{figure}



\begin{table*}[]
\begin{tabular}[t]{| c || c | c | c || c | c | c || c | c |}
\hline
& \multicolumn{3}{c||}{Heptagon} &  \multicolumn{3}{c||}{Reduced-rate SCF}& \multicolumn{2}{c|}{HaPPY Zero Rate } \\
  \hline
Radius & $n$ & $d^{(B)}$ & $d^{(W)}$ & $n$ & $d^{(B)}$  & $d^{(W)}$ &  $n$ & $d^{(B)}$ \\
\hline
1 & 7 & 3 & 3 & 5 &2 & 2 & 5 & 3\\
\hline
2 & 42 & 9 & 6 & 25 & 4 & 4 & 25 & 9\\
\hline
3 & 203 & 19 & 8 & 75 & 8 & 4 & 95 & 19\\
\hline
4 & 973 & 45 & 15 & 255 & 16 & 8 & 355 & 41\\
\hline
5 & 4662 & 99 & 29 & 745 & 20 & 8 & 1325 & 91\\
\hline
6 & 22337 & 221 & 80 & 2525 & 40 & 16 & 4945 & 321\\
\hline
Asymptotic& $\sim(5+\sqrt{21})^R$ & $\sim n^{0.54\pm0.03}$ & $\sim n^{0.37\pm0.07}$ & $\sim (5+2\sqrt{6})^{R}$ & $\sim n^{0.31\pm0.10}$ & $\sim n^{0.48\pm0.07}$& $\sim(2+\sqrt{3})^R$& $\sim n^{0.65\pm0.08}$ \\
\hline
%Exponent $0.95$ Confidence Intervals&&$0.51-0.56$&$0.30-0.43$&& $0.21-0.41$ & $0.42-0.55$& & $0.57-0.73$\\
%\hline
\end{tabular}
\caption{Numerically optimised bit and word distance of central logical qubits, with the $95\%$ confidence interval, as a function of radius to the boundary qubits. Additionally we show the asymptotic physical qubit count, $n$, as a function of the code radius, $R$, the code rate, $r$, and extrapolated power-law fits (the numerical prefactor is suppressed) to the numerically computed bit, $d^{(B)}$, and word, $d^{(W)}$, distances of the central logical qubit in each code family%dominant scaling term for number of qubits and the numeric fit of the distance for the each code
.}
\label{tab:distacetable}
\end{table*}

% \begin{table}[t!]
% \begin{tabular}[t]{| l || c |c | c | c | }
% \hline
%  Code Family & $n$ & $r\!=\!k/n$ & $d^{(B)}$  & $d^{(W)}$\\
%  \hline
% Max-rate Heptagon (Steane) & $((5\!+\!\sqrt{21})/2)^R$ & $0.22$ &  $ n^{0.54}$&  $ n^{0.37}$\\
% %Reduced-rate SCF ($R$ odd) & $ (5\!+\!2\sqrt{6})^{R}$ & $0.3$  &  $ n^{0.27}$&  $ n^{0.46}$\\
% Reduced-rate SCF ($R$ even) & $ (5\!+\!2\sqrt{6})^{R/2}$  & $0.09$ &  $ n^{0.30}$&  $ n^{0.50}$\\
% Zero-rate HaPPY  & $(2+\sqrt{3})^R$ & $0$ &  $ n^{0.65}$& --  \\
% \hline
% \end{tabular}
% \caption{.  % as a function of radius to the boundary qubits. Additionally we show the dominant scaling term for number of qubits and the numeric fit of the distance for the each code.
% }
% \label{tab:distacetable}
% \end{table}



%For example, the distances of the central logical qubit in a radius 2 code is the same as the logical qubit positioned at radius 2 in a radius 3 code, or any logical qubit on the penultimate boundary layer for any code size.

%It is also notable here that the distance measure equally applies to bulk qubits a defined depth from the boundary in an arbitary sized code. For example, regardless of code size the outer bulk qubits, depth 1 from the boundary, have the same distance as the central logical qubit in radius 1.




%\section{Conclusion}

\emph{Conclusions} We have developed a general purpose decoder for stabiliser codes, based on  integer optimisation.  Using this decoder, we have estimated thresholds against IID depolarising noise for different families of holographic codes, and shown that there is a tradeoff between the threshold and the code rate.  The moderately high thresholds against phenomenological depolarising noise are comparable to the surface code, together with finite rates,  may offer an alternative  for building quantum processors, however the development of an efficient decoder that also has thresholds is essential for implementation. The holographic code stabilisers  are non-local, so present challenges in implementation, however generating these codes with low-valence, local cluster states is the subject of ongoing work. %Because of these two things the holographic code is a promising finite rate alternative to the surface code worthy of further research. 
%
%The decoder described here is computationally expensive making it impractical for use experimentally. %does not have a suitable scaling for practical use, 
%However, the demonstration of reasonably high thresholds suggest that these codes may be practically interesting. %is useful to to filter promising error correcting codes.  
%The thresholds shown here, combined with the rate and low valence cluster state representation \cite{Harris2018, Mcmahon2020} show that the heptagon code may be a practical error correction code for future experimental use.

%\textcolor{red}{
%The high erasure threshold and code rate suggest that the heptagon code might be an attractive candidate for a practical error correcting code in networks that have weak geometric constraints, such as optical architectures \cite{Rudolph2017}.  Its performance against other logical error channels is the subject of ongoing research.  Further, since it is of CSS form, the heptagon code can be constructed from measurements on a suitably prepared cluster state \cite{Bolt2016}.  However, because some stabilisers have relatively large weight, the cluster states resulting from that construction would usually be high-valence, which tends to amplify imperfections during cluster creation.  We note here that the heptagon holographic code can be implemented with a low-valence cluster state; details will be reported in a forthcoming publication.  
%}

%\textcolor{red}{
%To conclude, we have developed the notion of block perfect tensors, a less restricted class than the perfect tensors introduced in earlier work.  This makes  a range of other codes available for tessellation in a  holographic tensor network, including the self-dual CSS Steane code, with which we have exemplified the general construction.  %\textcolor{red}{
%The stabilisers have a spectrum of weights, with most stabilisers being local and low weight, and proportionally fewer having larger weights.  As such, they may be suitable for cluster-state based measurement protocols \cite{Bolt2016}.}
%
%\textcolor{red}{
%Finally, we have applied a straightforward, optimal erasure decoder based on matrix row reduction on filtered support vectors to characterise the performance of holographic codes, yielding promising thresholds.  
%}



\begin{acknowledgements}
We thank Stephen Wright, Fred Roosta-Khorasani and David Poulin for useful discussions. 
This work was supported by the Australian Research Council Centre of Excellence for Engineered Quantum Systems (Grant No. CE 170100009), and the Asian Office of Aerospace Research and Development (AOARD) grant FA2386-18-1-4027.
\end{acknowledgements}

  \bibliography{ErrorCorrection,misc}

  \appendix
  \section{Appendix}
  
  We now briefly mention the uncertainties in our analysis. For the failure probability for fixed weight $P_{\textrm{failure}}$, we estimate the uncertainty in the results as
  \begin{equation}
      \sigma = \sqrt{\frac{P_{\textrm{failure}}(1-P_{\textrm{failure}})}{m}},
      \label{eq:error}
  \end{equation}
  where $m$ is the number of samples. In figure \ref{fig:ErrorGraphs} we show the estimate $P_{\textrm{failure}}$ for the max-rate heptagon code with radii $2-4$, along with error bars calulated using equation \ref{eq:error}.
  
  \begin{figure*}[t]
  \includegraphics[clip,width=0.32\columnwidth]{ErrorR2.pdf}
  \includegraphics[clip,width=0.32\columnwidth]{ErrorR3.pdf}
  \includegraphics[clip,width=0.32\columnwidth]{ErrorR4.pdf}
	
	\caption{Failure probability of the central logical qubit, with error bars, in the max-rate Heptagon code for radius a) $R=2$, b) $R=3$ and c) $R=4$, in the presence of a depolarising channel of fixed weight $\textrm{wt}(\varepsilon)$. 
	\label{fig:ErrorGraphs} }
\end{figure*}


